any4: Learned 4-bit Numeric Representation for LLMs

We present any4, a learned 4-bit weight quantization solution for large language models (LLMs) providing arbitrary numeric representations without requiring pre-processing of weights or activations. any4 yields higher accuracy compared to other related 4-bit numeric representation types: int4, fp4 and nf4, as evaluated on a range of model sizes, generations and families (Llama 2, Llama 3, Mistral and Mixtral). While any4 does not require preprocessing of weights or activations, it is also competitive with orthogonal techniques that require such preprocessing (e.g., AWQ and GPTQ). We also experiment with any3 and any2 and show competitiveness at lower bits. Additionally, we show that we can calibrate using a single curated diverse sample rather than hundreds of samples from a dataset as done in most quantization approaches. We also open source tinygemm, a latency optimized GPU matrix multiplication library for LLMs, that implements any4 using a GPU-efficient lookup table strategy along with other common quantization methods. We open source our code at https://github.com/facebookresearch/any4 .

==> tables/numeric-formats/llama2-13b.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{tabular}{l
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r }
\toprule
\multicolumn{11}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama2 13B}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\
\midrule
                             & \multicolumn{4}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                                                                                                                                                      & \multicolumn{6}{c}{\cellcolor[HTML]{C9DAF8}\textbf{Tasks ↑}}                                                                                                                                                                                                                                                                                                                                                                                                                            \\
\multirow{-2}{*}{}           & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{PTB}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{CodeParrot}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}HumanEval\\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}MBPP \\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{MMLU}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{HellaSwag}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{GSM8K}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{BigBench}} \\
\midrule
\cellcolor[HTML]{CCCCCC}FP16 & \cellcolor[HTML]{CCCCCC}4.88                                    & \cellcolor[HTML]{CCCCCC}6.47                            & \cellcolor[HTML]{CCCCCC}28.93                            & \cellcolor[HTML]{CCCCCC}2.40                                    & \cellcolor[HTML]{CCCCCC}19.5\%                                                                                  & \cellcolor[HTML]{CCCCCC}18.4\%                                                                              & \cellcolor[HTML]{CCCCCC}50.5\%                            & \cellcolor[HTML]{CCCCCC}60.0\%                                 & \cellcolor[HTML]{CCCCCC}23.2\%                             & \cellcolor[HTML]{CCCCCC}47.4\%                                \\
INT4                         & 5.05                                                            & 6.65                                                    & 30.79                                                    & 2.45                                                            & 15.2\%                                                                                                          & 16.4\%                                                                                                      & 48.8\%                                                    & 59.3\%                                                         & 20.8\%                                                     & 44.2\%                                                        \\
FP4                          & 5.07                                                            & 6.67                                                    & 30.96                                                    & 2.46                                                            & 15.2\%                                                                                                          & 16.2\%                                                                                                      & 49.5\%                                                    & 59.3\%                                                         & 19.3\%                                                     & 43.0\%                                                        \\
NF4                          & 4.99                                                            & 6.58                                                    & 31.17                                                    & 2.43                                                            & \textbf{15.9\%}                                                                                                 & 16.0\%                                                                                                      & \textbf{49.9\%}                                           & \textbf{59.9\%}                                                & \textbf{22.1\%}                                            & \textbf{44.6\%}                                               \\
ANY4                         & \textbf{4.97}                                                   & \textbf{6.55}                                           & \textbf{28.83}                                           & \textbf{2.42}                                                   & 15.2\%                                                                                                          & \textbf{18.0\%}                                                                                             & 49.3\%                                                    & 59.5\%                                                         & 21.6\%                                                     & \textbf{44.6\%}                                              \\
\bottomrule
\end{tabular}



==> tables/numeric-formats/llama2-70b.tex <==
\begin{tabular}{l
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r }
\toprule
\multicolumn{11}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama2 70B}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\
\midrule
                             & \multicolumn{4}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                                                                                                                                                      & \multicolumn{6}{c}{\cellcolor[HTML]{C9DAF8}\textbf{Tasks ↑}}                                                                                                                                                                                                                                                                                                                                                                                                                            \\
\multirow{-2}{*}{}           & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{PTB}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{CodeParrot}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}HumanEval\\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}MBPP \\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{MMLU}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{HellaSwag}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{GSM8K}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{BigBench}} \\
\midrule
\cellcolor[HTML]{CCCCCC}FP16 & \cellcolor[HTML]{CCCCCC}3.32                                    & \cellcolor[HTML]{CCCCCC}5.52                            & \cellcolor[HTML]{CCCCCC}14.44                            & \cellcolor[HTML]{CCCCCC}2.11                                    & \cellcolor[HTML]{CCCCCC}31.7\%                                                                                  & \cellcolor[HTML]{CCCCCC}37.4\%                                                                              & \cellcolor[HTML]{CCCCCC}65.2\%                            & \cellcolor[HTML]{CCCCCC}64.8\%                                 & \cellcolor[HTML]{CCCCCC}53.3\%                             & \cellcolor[HTML]{CCCCCC}67.1\%                                \\
INT4                         & 3.46                                                            & 5.61                                                    & 14.71                                                    & 2.14                                                            & 26.8\%                                                                                                          & \textbf{37.8\%}                                                                                             & 64.4\%                                                    & \textbf{64.7\%}                                                & 51.4\%                                                     & 65.0\%                                                        \\
FP4                          & 3.53                                                            & 5.67                                                    & 14.34                                                    & 2.16                                                            & 28.0\%                                                                                                          & 30.6\%                                                                                                      & 64.1\%                                                    & 64.0\%                                                         & \textbf{51.6\%}                                            & 65.0\%                                                        \\
NF4                          & 3.44                                                            & 5.61                                                    & 14.65                                                    & 2.14                                                            & \textbf{29.9\%}                                                                                                 & 37.2\%                                                                                                      & 64.5\%                                                    & 63.9\%                                                         & 50.6\%                                                     & 65.4\%                                                        \\
ANY4                         & \textbf{3.40}                                                   & \textbf{5.58}                                           & \textbf{14.64}                                           & \textbf{2.13}                                                   & 26.8\%                                                                                                          & 35.8\%                                                                                                      & \textbf{64.8\%}                                           & 64.5\%                                                         & \textbf{51.6\%}                                            & \textbf{66.6\%}                                              \\
\bottomrule
\end{tabular}

==> tables/numeric-formats/llama2-7b.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{tabular}{l
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r }
\toprule
\multicolumn{11}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama2 7B}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\
\midrule
                             & \multicolumn{4}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                                                                                                                                                      & \multicolumn{6}{c}{\cellcolor[HTML]{C9DAF8}\textbf{Tasks ↑}}                                                                                                                                                                                                                                                                                                                                                                                                                            \\
\multirow{-2}{*}{}           & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{PTB}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{CodeParrot}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}HumanEval\\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}MBPP \\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{MMLU}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{HellaSwag}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{GSM8K}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{BigBench}} \\
\midrule
\cellcolor[HTML]{CCCCCC}FP16 & \cellcolor[HTML]{CCCCCC}5.47                                    & \cellcolor[HTML]{CCCCCC}6.97                            & \cellcolor[HTML]{CCCCCC}20.83                            & \cellcolor[HTML]{CCCCCC}2.54                                    & \cellcolor[HTML]{CCCCCC}17.1\%                                                                                  & \cellcolor[HTML]{CCCCCC}20.0\%                                                                              & \cellcolor[HTML]{CCCCCC}41.3\%                            & \cellcolor[HTML]{CCCCCC}57.2\%                                 & \cellcolor[HTML]{CCCCCC}13.6\%                             & \cellcolor[HTML]{CCCCCC}39.8\%                                \\
INT4                         & 5.74                                                            & 7.30                                                    & 24.00                                                    & 2.63                                                            & 10.4\%                                                                                                          & 18.2\%                                                                                                      & 38.1\%                                                    & 56.4\%                                                         & 10.6\%                                                     & 36.5\%                                                        \\
FP4                          & 5.83                                                            & 7.37                                                    & 22.57                                                    & 2.65                                                            & 11.0\%                                                                                                          & 16.8\%                                                                                                      & 36.5\%                                                    & 56.6\%                                                         & 11.2\%                                                     & 35.5\%                                                        \\
NF4                          & 5.66                                                            & 7.19                                                    & 22.82                                                    & 2.60                                                            & 11.6\%                                                                                                          & \textbf{19.2\%}                                                                                             & 37.4\%                                                    & \textbf{56.8\%}                                                & 12.0\%                                                     & 36.8\%                                                        \\
ANY4                         & \textbf{5.59}                                                   & \textbf{7.10}                                           & \textbf{21.23}                                           & \textbf{2.57}                                                   & \textbf{14.0\%}                                                                                                 & 18.4\%                                                                                                      & \textbf{40.3\%}                                           & 56.7\%                                                         & \textbf{12.7\%}                                            & \textbf{36.9\%}                                              \\
\bottomrule
\end{tabular}



==> tables/numeric-formats/llama3-70b.tex <==
\begin{tabular}{l
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r }
%\toprule
\multicolumn{11}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama3 70B}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\
\midrule
                             & \multicolumn{4}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                                                                                                                                                      & \multicolumn{6}{c}{\cellcolor[HTML]{C9DAF8}\textbf{Tasks ↑}}                                                                                                                                                                                                                                                                                                                                                                                                                            \\
\multirow{-2}{*}{}           & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{PTB}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{CodeParrot}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}HumanEval\\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}MBPP \\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{MMLU}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{HellaSwag}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{GSM8K}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{BigBench}} \\
\midrule
\cellcolor[HTML]{CCCCCC}FP16 & \cellcolor[HTML]{CCCCCC}2.86                                    & \cellcolor[HTML]{CCCCCC}6.77                            & \cellcolor[HTML]{CCCCCC}8.16                             & \cellcolor[HTML]{CCCCCC}1.91                                    & \cellcolor[HTML]{CCCCCC}17.7\%                                                                                  & \cellcolor[HTML]{CCCCCC}60.8\%                                                                              & \cellcolor[HTML]{CCCCCC}75.4\%                            & \cellcolor[HTML]{CCCCCC}66.3\%                                 & \cellcolor[HTML]{CCCCCC}80.6\%                             & \cellcolor[HTML]{CCCCCC}82.4\%                                \\
INT4                         & 3.63                                                            & 7.97                                                    & 8.86                                                     & 2.21                                                            & 18.3\%                                                                                                          & 45.0\%                                                                                                      & 73.0\%                                                    & \textbf{66.2\%}                                                & 73.9\%                                                     & 78.4\%                                                        \\
FP4                          & 3.94                                                            & 7.76                                                    & 8.99                                                     & 2.17                                                            & \textbf{22.0\%}                                                                                                 & 50.8\%                                                                                                      & 71.9\%                                                    & 65.6\%                                                         & 75.3\%                                                     & 77.9\%                                                        \\
NF4                          & 3.43                                                            & 7.67                                                    & 8.84                                                     & 2.15                                                            & 18.9\%                                                                                                          & 39.6\%                                                                                                      & 73.7\%                                                    & 66.1\%                                                         & 75.9\%                                                     & 79.3\%                                                        \\
ANY4                         & \textbf{3.20}                                                   & \textbf{7.01}                                           & \textbf{8.33}                                            & \textbf{1.99}                                                   & 17.1\%                                                                                                          & \textbf{57.4\%}                                                                                             & \textbf{75.1\%}                                           & 66.1\%                                                         & \textbf{78.5\%}                                            & \textbf{81.8\%}                                              \\
\bottomrule
\end{tabular}


==> tables/numeric-formats/llama3-8b.tex <==
\begin{tabular}{l
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r }
%\toprule
\multicolumn{11}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama3 8B}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\
\midrule
                             & \multicolumn{4}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                                                                                                                                                      & \multicolumn{6}{c}{\cellcolor[HTML]{C9DAF8}\textbf{Tasks ↑}}                                                                                                                                                                                                                                                                                                                                                                                                                            \\
\multirow{-2}{*}{}           & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{PTB}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{CodeParrot}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}HumanEval\\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}MBPP \\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{MMLU}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{HellaSwag}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{GSM8K}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{BigBench}} \\
\midrule
\cellcolor[HTML]{CCCCCC}FP16 & \cellcolor[HTML]{CCCCCC}6.14                                    & \cellcolor[HTML]{CCCCCC}8.93                            & \cellcolor[HTML]{CCCCCC}10.59                            & \multicolumn{1}{r}{\cellcolor[HTML]{CCCCCC}2.54}                    & \cellcolor[HTML]{CCCCCC}29.3\%                                                                                  & \cellcolor[HTML]{CCCCCC}41.4\%                                                                              & \cellcolor[HTML]{CCCCCC}62.0\%                            & \cellcolor[HTML]{CCCCCC}60.1\%                                 & \cellcolor[HTML]{CCCCCC}50.7\%                             & \cellcolor[HTML]{CCCCCC}62.8\%                                \\
INT4                         & 6.87                                                            & 9.89                                                    & 11.37                                                    & 2.83                                                            & 23.2\%                                                                                                          & 35.4\%                                                                                                      & 59.6\%                                                    & 58.6\%                                                         & 40.6\%                                                     & 58.5\%                                                        \\
FP4                          & 7.10                                                            & 10.22                                                   & 11.81                                                    & 2.89                                                            & 22.0\%                                                                                                          & 36.8\%                                                                                                      & 57.1\%                                                    & 58.5\%                                                         & 35.0\%                                                     & 53.2\%                                                        \\
NF4                          & 6.63                                                            & 9.52                                                    & 11.14                                                    & 2.72                                                            & \textbf{23.2\%}                                                                                                 & \textbf{39.2\%}                                                                                             & 60.7\%                                                    & 59.1\%                                                         & 41.1\%                                                     & 59.0\%                                                        \\
ANY4                         & \textbf{6.51}                                                   & \textbf{9.40}                                           & \textbf{11.07}                                           & \textbf{2.68}                                                   & 21.3\%                                                                                                          & \textbf{39.2\%}                                                                                             & \textbf{61.0\%}                                           & \textbf{59.5\%}                                                & \textbf{41.7\%}                                            & \textbf{59.2\%}                                              \\
\bottomrule
\end{tabular}



==> tables/numeric-formats/llama3.2-1b.tex <==
\begin{tabular}{l
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r }
\toprule
\multicolumn{11}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama3.2 1B}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\
\midrule
                             & \multicolumn{4}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                                                                                                                                                      & \multicolumn{6}{c}{\cellcolor[HTML]{C9DAF8}\textbf{Tasks ↑}}                                                                                                                                                                                                                                                                                                                                                                                                                            \\
\multirow{-2}{*}{}           & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{PTB}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{CodeParrot}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}HumanEval\\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{\begin{tabular}[c]{@{}c@{}}MBPP \\ Pass@1\end{tabular}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{MMLU}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{HellaSwag}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{GSM8K}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{BigBench}} \\
\midrule
\cellcolor[HTML]{CCCCCC}FP16 & \cellcolor[HTML]{CCCCCC}9.76                                    & \cellcolor[HTML]{CCCCCC}12.77                           & \cellcolor[HTML]{CCCCCC}16.56                            & \cellcolor[HTML]{CCCCCC}3.49                                    & \cellcolor[HTML]{CCCCCC}16.46\%                                                                                 & \cellcolor[HTML]{CCCCCC}21.4\%                                                                              & \cellcolor[HTML]{CCCCCC}36.1\%                            & \cellcolor[HTML]{CCCCCC}47.7\%                                 & \cellcolor[HTML]{CCCCCC}6.60\%                             & \cellcolor[HTML]{CCCCCC}31.1\%                                \\
INT4                         & 11.89                                                           & 15.74                                                   & 20.32                                                    & 4.08                                                            & 9.76\%                                                                                                          & 11.4\%                                                                                                      & 30.1\%                                                    & 44.7\%                                                         & 3.18\%                                                     & 26.2\%                                                        \\
FP4                          & 13.01                                                           & 17.11                                                   & 21.89                                                    & 4.28                                                            & 8.54\%                                                                                                          & 5.8\%                                                                                                       & 29.3\%                                                    & 43.6\%                                                         & 2.27\%                                                     & 23.3\%                                                        \\
NF4                          & 10.99                                                           & 14.63                                                   & 18.78                                                    & 3.82                                                            & \textbf{13.4\%}                                                                                                 & \textbf{13.8\%}                                                                                             & \textbf{33.3\%}                                           & 45.8\%                                                         & 2.65\%                                                     & 26.8\%                                                        \\
ANY4                         & \textbf{10.63}                                                  & \textbf{13.95}                                          & \textbf{17.94}                                           & \textbf{3.71}                                                   & 11.0\%                                                                                                          & \textbf{18.6\%}                                                                                             & 32.9\%                                                    & \textbf{46.7\%}                                                & \textbf{3.71\%}                                            & \textbf{29.0\%}                                              \\
\bottomrule
\end{tabular}


==> tables/numeric-formats/mistral-7b-instructv0.2.tex <==
\begin{tabular}{l
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r }
\toprule
\multicolumn{9}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Mistral-7B Instruct v0.2}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\
\midrule
                             & \multicolumn{4}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                                                                                                                                                      & \multicolumn{4}{c}{\cellcolor[HTML]{C9DAF8}\textbf{Tasks ↑}}                                                                                                                                                                                            \\
\multirow{-2}{*}{}           & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{PTB}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{CodeParrot}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{MMLU}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{HellaSwag}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{GSM8K}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{BigBench}} \\
\midrule
\cellcolor[HTML]{CCCCCC}FP16 & \cellcolor[HTML]{CCCCCC}5.95                                    & \cellcolor[HTML]{CCCCCC}8.82                            & \cellcolor[HTML]{CCCCCC}21.77                            & \cellcolor[HTML]{CCCCCC}2.63                                    & \cellcolor[HTML]{CCCCCC}58.7\%                            & \cellcolor[HTML]{CCCCCC}66.1\%                                 & \cellcolor[HTML]{CCCCCC}41.7\%                             & \cellcolor[HTML]{CCCCCC}\textbf{51.7\%}                       \\
INT4                         & 6.14                                                            & 9.03                                                    & 22.02                                                    & 2.70                                                            & 57.1\%                                                    & 65.1\%                                                         & 39.7\%                                                     & 50.4\%                                                        \\
FP4                          & 6.19                                                            & 9.10                                                    & 21.62                                                    & 2.70                                                            & 56.6\%                                                    & 64.7\%                                                         & 38.2\%                                                     & 47.7\%                                                        \\
NF4                          & 6.06                                                            & 8.93                                                    & 24.72                                                    & 2.66                                                            & 58.0\%                                                    & \textbf{65.5\%}                                                & 38.5\%                                                     & \textbf{51.8\%}                                               \\
ANY4                         & \textbf{6.00}                                                   & \textbf{8.85}                                           & \textbf{23.24}                                           & \textbf{2.64}                                                   & \textbf{58.6\%}                                           & 65.4\%                                                         & \textbf{41.1\%}                                            & \textbf{51.7\%}                                              \\
\bottomrule
\end{tabular}

==> tables/numeric-formats/mixtral-8x7b-instructv0.1.tex <==
\begin{tabular}{l
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r 
>{\columncolor[HTML]{C9DAF8}}r }
\toprule
\multicolumn{9}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Mixtral-8x7B Instruct v0.1}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\
\midrule
                             & \multicolumn{4}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                                                                                                                                                      & \multicolumn{4}{c}{\cellcolor[HTML]{C9DAF8}\textbf{Tasks ↑}}                                                                                                                                                                                            \\
\multirow{-2}{*}{}           & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{PTB}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{CodeParrot}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{MMLU}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{HellaSwag}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{GSM8K}} & \multicolumn{1}{c}{\cellcolor[HTML]{C9DAF8}\textbf{BigBench}} \\
\midrule
\cellcolor[HTML]{CCCCCC}FP16 & \cellcolor[HTML]{CCCCCC}4.14                                    & \cellcolor[HTML]{CCCCCC}7.18                            & \cellcolor[HTML]{CCCCCC}16.47                            & \cellcolor[HTML]{CCCCCC}2.20                                    & \cellcolor[HTML]{CCCCCC}68.2\%                            & \cellcolor[HTML]{CCCCCC}67.6\%                                 & \cellcolor[HTML]{CCCCCC}64.8\%                             & \cellcolor[HTML]{CCCCCC}68.1\%                                \\
INT4                         & 4.45                                                            & 7.45                                                    & 16.84                                                    & 2.26                                                            & 66.5\%                                                    & 66.3\%                                                         & 57.8\%                                                     & 61.8\%                                                        \\
FP4                          & 4.46                                                            & 7.48                                                    & 18.42                                                    & 2.27                                                            & 66.8\%                                                    & 66.5\%                                                         & 59.4\%                                                     & 62.8\%                                                        \\
NF4                          & 4.30                                                            & 7.32                                                    & \textbf{15.00}                                           & 2.24                                                            & 67.6\%                                                    & 67.2\%                                                         & 61.0\%                                                     & 66.5\%                                                        \\
ANY4                         & \textbf{4.27}                                                   & \textbf{7.27}                                           & 16.14                                                    & \textbf{2.22}                                                   & 67.7\%                                                    & 67.1\%                                                         & 62.8\%                                                     & 65.8\%                                                       \\
\bottomrule
\end{tabular}



==> tables/quantization-algorithms/llama2-13b-lower-bits.tex <==
\begin{tabular}{cll
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r }
\toprule
\multicolumn{5}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama2 13B}}                                                                                                                                                                                                          \\
\midrule
\multicolumn{1}{l}{}                         &                                           &                                                   & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                         \\
\multicolumn{1}{l}{\multirow{-2}{*}{}}       & \multirow{-2}{*}{\textbf{\shortstack{Numeric \\ Format}}} & \multirow{-2}{*}{\textbf{\shortstack{Quantization \\ Algorithm}}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} \\
\midrule
\multicolumn{1}{l}{\cellcolor[HTML]{CCCCCC}} & \cellcolor[HTML]{CCCCCC}FP16              & \cellcolor[HTML]{CCCCCC}                          & \cellcolor[HTML]{CCCCCC}4.88                                    & \cellcolor[HTML]{CCCCCC}6.47                            \\
                                             & INT3                                      & RTN                                               & 6.13                                                            & 7.99                                                    \\
                                             & INT3                                      & GPTQ                                              & 5.31                                                            & 7.06                                                    \\
                                             & INT3                                      & AWQ                                               & \textbf{5.32}                                                   & 6.94                                                    \\
\multirow{-4}{*}{\textbf{3-bits}}            & ANY3                                      & RTN                                               & 5.34                                                            & \textbf{6.90}                                          \\
\bottomrule
\end{tabular}



==> tables/quantization-algorithms/llama2-13b.tex <==
\begin{tabular}{cll
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r }
\toprule
\multicolumn{5}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama2 13B}}                                                                                                                                                                                                          \\
\midrule
\multicolumn{1}{l}{}                         &                                           &                                                   & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                         \\
\multicolumn{1}{l}{\multirow{-2}{*}{}}       & \multirow{-2}{*}{\textbf{\shortstack{Numeric \\ Format}}} & \multirow{-2}{*}{\textbf{\shortstack{Quantization \\ Algorithm}}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} \\
\midrule
\multicolumn{1}{l}{\cellcolor[HTML]{CCCCCC}} & \cellcolor[HTML]{CCCCCC}FP16              & \cellcolor[HTML]{CCCCCC}                          & \cellcolor[HTML]{CCCCCC}4.88                                    & \cellcolor[HTML]{CCCCCC}6.47                            \\
                                             & INT4                                      & RTN                                               & 5.05                                                            & 6.65                                                    \\
                                             & INT4                                      & GPTQ                                              & 4.96                                                            & 6.57                                                    \\
                                             & INT4                                      & AWQ                                               & \textbf{4.97}                                                   & 6.56                                                    \\
                                             & ANY4                                      & RTN                                               & \textbf{4.97}                                                   & \textbf{6.55}                                           \\
                                             & ANY4                                      & GPTQ                                              & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}TBD}                                                                           \\
\multirow{-6}{*}{\textbf{4-bits}}            & \textbf{ANY4}                             & \textbf{AWQ}                                      & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}TBD}                                                                          \\
\bottomrule
\end{tabular}

==> tables/quantization-algorithms/llama2-70b-lower-bits.tex <==
\begin{tabular}{cll
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r }
\toprule
\multicolumn{5}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama2 70B}}                                                                                                                                                                                                          \\
\midrule
\multicolumn{1}{l}{}                         &                                           &                                                   & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                         \\
\multicolumn{1}{l}{\multirow{-2}{*}{}}       & \multirow{-2}{*}{\textbf{\shortstack{Numeric \\ Format}}} & \multirow{-2}{*}{\textbf{\shortstack{Quantization \\ Algorithm}}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} \\
\midrule
\multicolumn{1}{l}{\cellcolor[HTML]{CCCCCC}} & \cellcolor[HTML]{CCCCCC}FP16              & \cellcolor[HTML]{CCCCCC}                          & \cellcolor[HTML]{CCCCCC}3.32                                    & \cellcolor[HTML]{CCCCCC}5.52                            \\
                                             & INT3                                      & RTN                                               & 4.45                                                            & 6.58                                                    \\
                                             & INT3                                      & GPTQ                                              & 3.88                                                            & 5.87                                                    \\
                                             & INT3                                      & AWQ                                               & 3.74                                                            & 5.81                                                    \\
\multirow{-4}{*}{\textbf{3-bits}}            & ANY3                                      & RTN                                               & \textbf{3.73}                                                   & \textbf{5.80}                                          \\
\bottomrule
\end{tabular}



==> tables/quantization-algorithms/llama2-70b.tex <==
\begin{tabular}{cll
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r }
\toprule
\multicolumn{5}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama2 70B}}                                                                                                                                                                                                          \\
\midrule
\multicolumn{1}{l}{}                         &                                           &                                                   & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                         \\
\multicolumn{1}{l}{\multirow{-2}{*}{}}       & \multirow{-2}{*}{\textbf{\shortstack{Numeric \\ Format}}} & \multirow{-2}{*}{\textbf{\shortstack{Quantization \\ Algorithm}}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} \\
\midrule
\multicolumn{1}{l}{\cellcolor[HTML]{CCCCCC}} & \cellcolor[HTML]{CCCCCC}FP16              & \cellcolor[HTML]{CCCCCC}                          & \cellcolor[HTML]{CCCCCC}3.32                                    & \cellcolor[HTML]{CCCCCC}5.52                            \\
                                             & INT4                                      & RTN                                               & 3.46                                                            & 5.61                                                    \\
                                             & INT4                                      & GPTQ                                              & 3.42                                                            & 5.59                                                    \\
                                             & INT4                                      & AWQ                                               & 3.41                                                            & \textbf{5.58}                                           \\
                                             & ANY4                                      & RTN                                               & \textbf{3.40}                                                   & \textbf{5.58}                                           \\
                                             & ANY4                                      & GPTQ                                              & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}TBD}                                                                           \\
\multirow{-6}{*}{\textbf{4-bits}}            & \textbf{ANY4}                             & \textbf{AWQ}                                      & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}TBD}                                                                          \\
\bottomrule
\end{tabular}


==> tables/quantization-algorithms/llama2-7b-lower-bits.tex <==
\begin{tabular}{cll
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r }
\toprule
\multicolumn{5}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama2 7B}}                                                                                                                                                                                                           \\
\midrule
\multicolumn{1}{l}{}                         &                                           &                                                   & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                         \\
\multicolumn{1}{l}{\multirow{-2}{*}{}}       & \multirow{-2}{*}{\textbf{\shortstack{Numeric \\ Format}}} & \multirow{-2}{*}{\textbf{\shortstack{Quantization \\ Algorithm}}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} \\
\midrule
\multicolumn{1}{l}{\cellcolor[HTML]{CCCCCC}} & \cellcolor[HTML]{CCCCCC}FP16              & \cellcolor[HTML]{CCCCCC}                          & \cellcolor[HTML]{CCCCCC}5.47                                    & \cellcolor[HTML]{CCCCCC}6.97                            \\
                                             & INT3                                      & RTN                                               & 8.70                                                            & 11.10                                                   \\
                                             & INT3                                      & GPTQ                                              & 6.25                                                            & 7.97                                                    \\
                                             & INT3                                      & AWQ                                               & 6.24                                                            & 7.84                                                    \\
\multirow{-4}{*}{\textbf{3-bits}}            & ANY3                                      & RTN                                               & \textbf{6.11}                                                   & \textbf{7.66}                                          \\
\bottomrule
\end{tabular}
        

==> tables/quantization-algorithms/llama2-7b.tex <==
\begin{tabular}{cll
>{\columncolor[HTML]{D9EAD3}}r 
>{\columncolor[HTML]{D9EAD3}}r }
\toprule
\multicolumn{5}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Llama2 7B}}                                                                                                                                                                                                           \\
\midrule
\multicolumn{1}{l}{}                         &                                           &                                                   & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}\textbf{Perplexity ↓}}                                                         \\
\multicolumn{1}{l}{\multirow{-2}{*}{}}       & \multirow{-2}{*}{\textbf{\shortstack{Numeric \\ Format}}} & \multirow{-2}{*}{\textbf{\shortstack{Quantization \\ Algorithm}}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{WikiText-2}} & \multicolumn{1}{c}{\cellcolor[HTML]{D9EAD3}\textbf{C4}} \\
\midrule
\multicolumn{1}{l}{\cellcolor[HTML]{CCCCCC}} & \cellcolor[HTML]{CCCCCC}FP16              & \cellcolor[HTML]{CCCCCC}                          & \cellcolor[HTML]{CCCCCC}5.47                                    & \cellcolor[HTML]{CCCCCC}6.97                            \\
                                             & INT4                                      & RTN                                               & 5.73                                                            & 7.30                                                    \\
                                             & INT4                                      & GPTQ                                              & 5.72                                                            & 7.23                                                    \\
                                             & INT4                                      & AWQ                                               & 5.72                                                            & 7.13                                                    \\
                                             & ANY4                                      & RTN                                               & \textbf{5.59}                                                   & \textbf{7.10}                                           \\
                                             & ANY4                                      & GPTQ                                              & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}TBD}                                                                           \\
\multirow{-6}{*}{\textbf{4-bits}}            & ANY4                                      & AWQ                                               & \multicolumn{2}{c}{\cellcolor[HTML]{D9EAD3}TBD}                                                                          \\
\bottomrule
\end{tabular}
    

